CsFEVER and CTKFacts: Acquiring Czech data for fact verification

In this paper, we examine several methods of acquiring Czech data for automated fact-checking, which is a task commonly modeled as a classification of textual claim veracity w.r.t. a corpus of trusted ground truths. We attempt to collect sets of data in form of a factual claim, evidence within the ground truth corpus, and its veracity label (supported, refuted or not enough info). As a first attempt, we generate a Czech version of the large-scale FEVER dataset built on top of Wikipedia corpus. We take a hybrid approach of machine translation and document alignment; the approach and the tools we provide can be easily applied to other languages. We discuss its weaknesses and inaccuracies, propose a future approach for their cleaning and publish the 127k resulting translations, as well as a version of such dataset reliably applicable for the Natural Language Inference task - the CsFEVER-NLI. Furthermore, we collect a novel dataset of 3,097 claims, which is annotated using the corpus of 2.2M articles of Czech News Agency. We present its extended annotation methodology based on the FEVER approach, and, as the underlying corpus is kept a trade secret, we also publish a standalone version of the dataset for the task of Natural Language Inference we call CTKFactsNLI. We analyze both acquired datasets for spurious cues - annotation patterns leading to model overfitting. CTKFacts is further examined for inter-annotator agreement, thoroughly cleaned, and a typology of common annotator errors is extracted. Finally, we provide baseline models for all stages of the fact-checking pipeline and publish the NLI datasets, as well as our annotation platform and other experimental data.

==> src/__latexindent_temp.tex <==
\section{Conclusion}\label{sec:conclusion}

With this paper, we aimed to address the lack of a Czech dataset for automated fact-checking.
We have explored two ways of acquiring such data.

Firstly, we localize the \FEN dataset, using a document alignment between Czech and English \Wikipedia abstracts extracted from the \textit{interlingual links}.
We obtain and publish the \FCZ dataset of 127k machine-translated claims with evidence enclosed within the Czech \Wikipedia dump.
We then validate our alignment scheme and measure a 66\% precision using hand annotations over a 1\% sample of obtained data.
Therefore, we recommend the data for models less sensitive to noise and utilize it to train experimental DR models and recall estimation.

Secondly, we execute a series of human annotation runs with 163 students of journalism to acquire a novel dataset in Czech.
As opposed to similar annotations that extracted the claims and evidence from \Wikipedia~\cite{fever2018,norregaard2021danfever,aly2021feverous}, we annotate our dataset on top of a CTK corpus extracted from a news agency archive to explore this different relevant language form. 
We collect a raw dataset of 3,116 labeled claims, 57\% of which have at $\geq2$ independent cross-annotations.
From these, we calculate Krippendorff's alpha to be 56.42\%.
We proceed with manual and human-and-model-in-the-loop annotation cleaning to remove conflict and malformed annotations and arrive at a thoroughly cleaned \CTK dataset of 3,097 claims and their veracity annotations with evidence from the CTK corpus.
We release its version for NLI called \CTKNLI to maintain corpus trade secrecy.

Finally, we use our datasets to train baseline models for the full fact-checking pipeline composed of Document Retrieval and Natural Language Inference tasks.
% At five retrieved paragraphs in a Score Evidence setting, where at least one gold set of evidence must be covered by the DR predictions, our best performing models scored 33.89\% overall accuracy on \FCZ and 20.14\% on \CTK.
% In a No Score Evidence setting, where the gold evidence requirement is removed, we scored 55.40\% and 61.24\% on \FCZ and \CTK, respectively.
% We claim the results to be testifying to the viability of the task in our setting and encouraging for further research on our data.

\subsection{Future work}
\begin{itemize}
    \item The fact-checking pipeline is to also be augmented by the \textit{check-worthiness estimation}~\cite{nakov2021automated}, that is, a model that classifies which sentences of a given text in Czech are appropriate for the fact verification.
    We are currently working on models that detect claims within the Czech Twitter, and a strong predictor for this task would also strengthen our annotation scheme from Section~\ref{sec:annotation} that currently relies on hand-picked check-worthy documents.
    \item While the \SUP, \REF{} and \NEI{} classes  offer a finer classification w.r.t. evidence than binary \texttt{true}/\texttt{false}, it is a good convention of fact-checking services to use additional labels, s.a. \texttt{MISINTERPRETED}, that could be integrated into the common automated fact verification scheme if well formalised.
    \item The enclosed annotation schemes for this task like that from~\cite{fever2018} or Section~\ref{sec:annotation} do not necessarily produce organic claims capturing the real-world complexity of fact-checking -- for example, just the \FEN \train set contains hundreds of claims of form \enquote{X is a person.}.
    This does not have a trivial solution, but we suggest an integration of real-world sources of claims, s.a. Twitter, into the annotation scheme.
    \item While the \FEVER localization scheme from Section~\ref{fcz-method} yielded a rather noisy dataset, its size and document precision encourage
    deployment of a model-based cleaning scheme like that from~\cite{Jeatrakul} to further refine its results.
\end{itemize}

==> src/licensing.tex <==
%!TEX ROOT=../lrec2021.tex

\section{Licensing}
\hu{Note this section is probably temporary and its contents will be distributed into appropriate previous sections once resolved. \todo{Remove}}

\hu{\url{https://ufal.mff.cuni.cz/~popel/npfl070/slides/authors_rights_intro.pdf} -- Good and easily digestible reading on the topics -- generally we want to use CC BY (\q{Attribution} -- citation required) + SA (\q{Share alike})}

\subsection{Licenses of used data}
Necessary to keep an eye on -- may be restrictive, so we may need to contact authors for an extra permission:

\begin{enumerate}
    \item DeepL translation -- we care about the \q{\textbf{processed content}} terms entity -- it mostly looks like free use as long as we give a DeepL company name and link, see: \url{https://www.deepl.com/pro-license/}

    \textit{All rights regarding the Content, Processed Content and/or Customer Training Data remain with Customer. However, Customer grants DeepL the non-exclusive worldwide right to use the Content and/or Customer Training Data solely in order to provide DeepL’s services to Customer. In particular, Customer grants to DeepL the right to temporarily store, modify, process, translate and transmit the Content and/or Customer Training Data, and to sublicense the foregoing rights to its subcontractors, to the extent required to provide the services set out in this Agreement}
    \item CTK dataset -- proprietary, need to discuss permission
    \begin{itemize}
        \item $\rightarrow$ for \CTKNLI, Herbert proposes some version of CC-BY-SA
        \item $\rightarrow$ maybe we could make a SQLite DR sandbox out of the permitted CTK articles? not for full reproducibility, just technical/debug convenience (sth like \texttt{ctk\_filtered10000.db}) 
    \end{itemize}
    \item \FEN{} -- CC-BY-SA 3.0 -- \url{https://s3-eu-west-1.amazonaws.com/fever.public/license.html}
    \begin{itemize}
        \item $\rightarrow$ \FCZ must be CC-BY-SA 3.0 
    \end{itemize}
    \item \FEVERNLI{} -- MIT License -- but must cite~\cite{nie2019combining} \url{https://github.com/easonnie/combine-FEVER-NSMN/blob/master/other_resources/nli_fever.md}
    \begin{itemize}
        \item $\rightarrow$ we can freely publish \FCZ-NLI under CC-BY-SA as long as we cite
    \end{itemize}
    \item NLI datasets: 
    \begin{itemize}
        \item SNLI CC-BY (\url{https://huggingface.co/datasets/snli}) $\rightarrow$ only attribution required
        \item ANLI CC-BY-NC (\url{https://github.com/facebookresearch/anli/blob/main/LICENSE}) $\rightarrow$ attribution and non-profit flag required
    \end{itemize}
\end{enumerate}

==> src/revision_note.tex <==
%!TEX ROOT=../lrec2021.tex
\revision{
\section*{Revision notes}\label{sec:revision_note}
\begin{enumerate}
  \item Proposed title changed from \q{\FCZ and \CTK: Czech datasets for fact verification} to \textbf{\q{\papertitle}} -- \textit{maybe too weak/underpromissing?}
  \item Switched first-author order -- this shouldn't make a factic difference, but neccessary for Herbert's PhD studies accreditation 
  \item \textbf{Abstract} would need a full rewrite -- avoid over- and underpromissing. \todo{once all sections are in place}
  \item Minor tweaks in language for better clarity
  \item \todo{relevant use-case for \FCZ has to be found and \q{marketed} in Section~\ref{sec:fevercs}}
  \item The points for chapters~\ref{sec:ctkfacts} and \ref{sec:fevercs} have been integrated \todo{my Section~\ref{sec:nli-baseline} is IMHO quite bad and needs to be heavily altered}
\end{enumerate}
}
\pagebreak

